AHA!: Facilitating AI Impact Assessment by Generating Examples of Harms

While demands for change and accountability for harmful AI consequences mount, foreseeing the downstream effects of deploying AI systems remains a challenging task. We developed AHA! (Anticipating Harms of AI), a generative framework to assist AI practitioners and decision-makers in anticipating potential harms and unintended consequences of AI systems prior to development or deployment. Given an AI deployment scenario, AHA! generates descriptions of possible harms for different stakeholders. To do so, AHA! systematically considers the interplay between common problematic AI behaviors as well as their potential impacts on different stakeholders, and narrates these conditions through vignettes. These vignettes are then filled in with descriptions of possible harms by prompting crowd workers and large language models. By examining 4113 harms surfaced by AHA! for five different AI deployment scenarios, we found that AHA! generates meaningful examples of harms, with different problematic AI behaviors resulting in different types of harms. Prompting both crowds and a large language model with the vignettes resulted in more diverse examples of harms than those generated by either the crowd or the model alone. To gauge AHA!'s potential practical utility, we also conducted semi-structured interviews with responsible AI professionals (N=9). Participants found AHA!'s systematic approach to surfacing harms important for ethical reflection and discovered meaningful stakeholders and harms they believed they would not have thought of otherwise. Participants, however, differed in their opinions about whether AHA! should be used upfront or as a secondary-check and noted that AHA! may shift harm anticipation from an ideation problem to a potentially demanding review problem. Drawing on our results, we discuss design implications of building tools to help practitioners envision possible harms.

==> sections/additional_analyses.tex <==
\begin{table}[]
\scriptsize
\begin{tabular}{@{}lp{1.4cm}lllll}
\toprule
\rowcolor[HTML]{EFEFEF} 
Scenario    
& \begin{tabular}[c]{@{}l@{}}Crowd mean \\ (standard error)\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}GPT-3 mean \\ (standard error)\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Crowd + GPT-3 \\ (standard  error)\end{tabular} 
& \begin{tabular}[c]{@{}l@{}}Crowd vs. GPT-3\end{tabular}                                     
& \begin{tabular}[c]{@{}l@{}}Crowd vs. \\ Combined\end{tabular}                               
& \begin{tabular}[c]{@{}l@{}}GPT-3 vs. \\ Combined\end{tabular}                               
\\ \midrule


\textbf{\begin{tabular}[c]{@{}l@{}}Comm. compl.\end{tabular}} & \begin{tabular}[c]{@{}l@{}}13.67 (0.83)\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}14.08 (0.68)\end{tabular}                     & 19.17                                                                                             & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}l@{}}t(22) = -0.38 p = .70 (n.s.)\end{tabular}} & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(22) = -4.42 p = .0002\end{tabular}}    & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(22) = -4.42 p = .0002\end{tabular}}    \\

\textbf{Content moder.}                                                 & \begin{tabular}[c]{@{}l@{}}13.92 (0.72)\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}12.92 (0.92)\end{tabular}                     & 18.46                                                                                             & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}l@{}}t(24) = 0.85 p = .40 (n.s.)\end{tabular}}  & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(24) = -3.73 p = .001\end{tabular}}     & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(24) = -4.13 p = .0004\end{tabular}}    \\

\textbf{Disease diag.}                                                  & \begin{tabular}[c]{@{}l@{}}8.23 (0.40)\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}7.65 (0.42)\end{tabular}                      & 11                                                                                                & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}l@{}}t(32) = 1.02 p = .32 (n.s.)\end{tabular}}  & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(32) = -4.58 p = 6.68e-05\end{tabular}} & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(32) = -5.42 p = 5.76e-06\end{tabular}} \\

\textbf{Hiring}                                                             & \begin{tabular}[c]{@{}l@{}}11.09 (0.46)\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}10.91 (0.64)\end{tabular}                     & 13.58                                                                                             & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}l@{}}t(21) = 0.23 p = .81 (n.s.)\end{tabular}}  & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(21) = -3.27 p = .003\end{tabular}}     & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(21) = -3.06 p = .006\end{tabular}}     \\

\textbf{Loan applic.}                                                   & \begin{tabular}[c]{@{}l@{}}9 (0.38)\end{tabular}                         & \begin{tabular}[c]{@{}l@{}}10.27 (0.56)\end{tabular}                     & 13.72                                                                                             & {\color[HTML]{9B9B9B} \begin{tabular}[c]{@{}l@{}}t(20) = -1.88 p = .08 (n.s.)\end{tabular}} & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(20) = -7.46 p = 3.38e-07\end{tabular}} & {\color[HTML]{9A0000} \begin{tabular}[c]{@{}l@{}}t(20) = -4.59 p = .0001\end{tabular}}    \\ \bottomrule
\end{tabular}
\caption{Paired t-test for means of numbers of unique codes generated by Crowd only, GPT-3 only, and Combined (Crowd + GPT-3). For all the scenarios, Crowd and GPT-3 combined generate significantly more unique codes together than either alone.}
\vspace{-8pt}
\label{table:complementarity}
\end{table}







\subsubsection{What are the distributions of harms across different generation sources and problematic outcomes?}

Disaggregating the generations further to examine the differences between sources of generation for different problematic outcomes, we again do not notice substantial differences between GPT-3 and crowds. Figure ~\ref{fig:distribution-fp-source-scenarios} shows the distribution of harms disaggregated by type of AI mistake and source of generation.



\begin{figure}[t]

\includegraphics[width=\linewidth]{figures/harm_distributions_source_fp_scenario.pdf}
\caption{Distribution of harms disaggregated by the type of generation source -- GPT-3 and Crowd and type of problematic outcome.} \label{fig:distribution-fp-source-scenarios}
\end{figure}


\begin{table*}[]
\begin{tabular}{lllll}
\hline
                                                                                                                          & \textbf{\begin{tabular}[c]{@{}l@{}}False \\ Positive \\ (Crowd vs. GPT-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}False\\ Negative\\ (Crowd vs. GPT-3)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Crowd\\ \\ (FP vs. FN)\end{tabular}}             & \textbf{\begin{tabular}[c]{@{}l@{}}GPT-3\\ \\ (FP vs. FN)\end{tabular}}                                    \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Communication \\ compliance\end{tabular}}} & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=697)\\ = 530.93\\ $p < .0001$\end{tabular}     & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=714)\\ = 438.58\\ $p < .0001$\end{tabular}   & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=715)\\ = 517.15\\ $p < .0001$\end{tabular} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=696)\\ = 457.29\\ $p < .0001$\end{tabular}} \\
\multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Content \\ moderation\end{tabular}}}                               & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=598)\\ = 233.97\\ $p < .0001$\end{tabular}     & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=589)\\ = 177.74\\ $p < .0001$\end{tabular}   & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=601)\\ = 165.34\\ $p < .0001$\end{tabular} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=586)\\ = 254.3\\ $p < .0001$\end{tabular}}  \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Disease\\ diagnosis\end{tabular}}}         & \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=569)\\ = 233.97\\ $p < .0001$\end{tabular}     & \begin{tabular}[c]{@{}l@{}}$\chi^2$(7, N=609)\\ = 695.97\\ $p < .0001$\end{tabular}   & \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=614)\\ = 540.16\\ $p < .0001$\end{tabular} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=564)\\ = 577.79\\ $p < .0001$\end{tabular}} \\
\multicolumn{1}{l|}{\textbf{Hiring}}                                                                                      & \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=596)\\ = 1276\\ $p < .0001$\end{tabular}       & \begin{tabular}[c]{@{}l@{}}$\chi^2$(5, N=609)\\ = 916.7\\ $p < .0001$\end{tabular}    & \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=640)\\ = 1429.6\\ $p < .0001$\end{tabular} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}$\chi^2$(6, N=565)\\ = 788.1\\ $p < .0001$\end{tabular}}  \\
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}Loan\\ application\end{tabular}}}          & \begin{tabular}[c]{@{}l@{}}$\chi^2$(5, N=476)\\ = 816.97\\ $p < .0001$\end{tabular}     & \begin{tabular}[c]{@{}l@{}}$\chi^2$(5, N=449)\\ = 579.33\\ $p < .0001$\end{tabular}   & \begin{tabular}[c]{@{}l@{}}$\chi^2$(5, N=456)\\ = 656.13\\ $p < .0001$\end{tabular} & {\color[HTML]{333333} \begin{tabular}[c]{@{}l@{}}$\chi^2$(5, N=469)\\ = 741.94\\ $p < .0001$\end{tabular}} \\ \hline
\end{tabular}
\caption{Distribution of harms disaggregated by the type of generation source -- GPT-3 and Crowd and type of problematic outcome. $\chi^2$ tests of the distributions of the types of harms for pairwise comparisons: Crowd vs. GPT-3 by type of problematic outcome (first two columns), and False Positive vs. False Negative by type of source (last two columns).}
\end{table*}


\begin{figure}[h]

\includegraphics[width=\linewidth]{figures/diversity_source_po.pdf}
\caption{Diversity of types of harms as measured by the number of unique codes generated by Crowd and GPT-3 for different scenarios and problematic outcomes.} \label{fig:diversity-fp-source-scenarios}
\end{figure}


\iffalse
\subsubsection{Does the introduction of various dimensions of problematic behavior increase the diversity of generated harms?}

We sought to understand whether the dimensions of problematic outcomes that we introduced (i.e., \em accumulated\em, \em egregious\em, \em harm conditioned \em) contributed to an increase in the diversity of harms that were generated for each stakeholder. For improved readability, we pick a single scenario (i.e., 
\em hiring\em) -- visualize its distributions and focus on the interpretation of the results for the selected scenario only. However, motivated readers can check the Appendix for analyses of the rest of the scenarios.

Figure~\ref{fig:diversity-hiring} depicts the additional unique codes that were obtained for different stakeholders by introducing the three problematic outcome dimensions. We compared the means of unique codes generated per stakeholder without and with each of the problematic dimensions. Table~\ref{table:diversity-hiring} shows that \textbf{all the added dimensions of problematic outcomes increased the diversity of the generated harms significantly}.


\begin{figure*}[h]
\centering
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring/hiring_accumulated_unq_codes.pdf}
\caption{Accumulated} 
\label{fig:unq-codes-acc}
\end{subfigure}
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring/hiring_egregious_unq_codes.pdf}
\caption{Egregious}\label{fig:unq-codes-egregious}
\end{subfigure}
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring/hiring_harm_conditioned_unq_codes.pdf}
\caption{Harm conditioned}\label{fig:unq-codes-harm_cond}
\end{subfigure}
\caption{Hiring scenario. Additional unique codes (i.e., diversity of harms) gained from the introduction of different problematic outcome dimensions. }

\label{fig:diversity-hiring}
\end{figure*}

\begin{table}[]

\begin{tabular}{@{}lllll@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Added problematic \\ outcome dimension\end{tabular} & t statistic & df & p-value                     & \begin{tabular}[c]{@{}l@{}}mean difference \\ in unique codes\end{tabular} \\ \midrule
\textbf{Accumulated}                                                           & -3.36       & 11 & {\color[HTML]{9A0000} .006} & -1.25                                                                      \\
\textbf{Egregious}                                                             & -3.71       & 11 & {\color[HTML]{9A0000} .003} & -1.66                                                                      \\
\textbf{Harm conditioned}                                                      & -4.30       & 11 & {\color[HTML]{9A0000} .001} & -2.08                                                                      \\ \bottomrule
\end{tabular}
\caption{Hiring scenario. Paired t-test for the differences between means of the total number of unique codes generated per stakeholder without and with the problematic outcome added as a dimension.}
\label{table:diversity-hiring}
\end{table}



%Crowd diversity is significantly correlated with the qualitative code, but GPT-3 generations are not.

\fi

\begin{figure*}
\centering
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring_fp.pdf}
\caption{False positive vs. false negative} 
\label{fig:distribution-fp-scenarios}
\end{subfigure}
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring_accumulated.pdf}
\caption{Accumulated vs. one-time}\label{fig:accumulated_scenarios}
\end{subfigure}
\begin{subfigure}[b]{.45\linewidth}
\includegraphics[width=\linewidth]{figures/hiring_egregious.pdf}
\caption{Egregious vs. not specified}\label{fig:egregious}
\end{subfigure}
\caption{Difference in the percentage of points of the number of harms generated for different problematic outcome dimensions across stakeholders for the \em hiring \em scenario. }
\label{fig:problematic_outcomes}
\end{figure*}

==> sections/experiments.tex <==
\subsection{Experimental Setup}
\label{section:experiments}

To evaluate \frameworkname{} we experimented with five hypothetical high-stakes binary classification scenarios differing in the AI system's purpose and inspired by real-world AI incidents: resource allocation (hiring and loan application), online moderation policy enforcement
(content moderation and communication compliance), and diagnostics (disease diagnosis).

\subsubsection{Crowdsourcing Experiment}

We recruited crowdworkers from the Clickworker crowdsourcing platform (www.clickworker.com). Crowdworkers were first presented with a consent form before proceeding with the task. Each crowdworker was then presented with four different vignettes generated for one of our five hypothetical scenarios. Vignettes were selected randomly from that scenario's corresponding ethical matrix until each vignette was filled out by three crowdworkers. After completing the task, workers were also prompted with demographic and background questions. Our crowdsourcing study was approved by our institution's IRB.

% We identified spammers through an attention check question and by manually checking their responses. We then remove and recollect generations for responses that look like obviously spams (i.e., keysmash) and fail the attention check question. A complete list of questions can be found in the Appendix section. 



% Universal Human Relevance System (UHRS)

%Figure \ref{fig:sample-task} depicts a sample task.  


%[How many people per cell?] [Figure X depicts a sample task.]

%[Which platform? How many participants? Demographics. How much were they paid? Which participants' data were retained for analyses?]

Across all of our experiments, we employed $105$ English speaking judges from North America.
%via Microsoft's internal crowdsourcing tool---known as the Universal Human Relevance System (UHRS)~\cite{gray2016crowd,chen2019more}---that allows easy task design and quality control.  
%
We capped the number of assessments per judge to X and to remove spammers and under-performing judges (and re-judge corresponding HITs), we used a mix of post-annotation, speed checks, and attention checks.
%
Judges were paid for all HITs they performed, even when identified as spammers, paying on average about \$15 (USD) per hour.
%
In total, 98 trusted judges participated in our tasks. In addition to the task, we also collected self-reported age (18-25: 17\%, 25-39: 49\%, 40-64: 31\%, 65+:2\%), experience with similar AI systems (with over 50\% of those answering this question saying they are slightly familiar or not familiar at all), and whether they believe to have experienced adverse impacts due to AI systems (with only ~15\% of those answering this question reporting to have been experiencing adverse impacts from AI systems). 


%\subsubsection{Procedure}

%[Demographic questionnaire? Other questions?] 


\subsubsection{GPT-3 Experiment}
We also experimented with generating harms for each of our five scenarios by prompting GPT-3. 
We used few-short learning with a Davinci model. We prompted the model with a vignette that included a scenario description and a set of manually created examples (one example per stakeholder), as illustrated in Figure \ref{fig:sample_vignette}. For each vignette (i.e., cell of the Ethical Matrix) we generated three different completions. 
%[How did we prompt GPT-3? How many generations per cell? What was the context provided? What was the exclusion criteria?]




==> sections/findings-chau.tex <==

Notes on themes: 
-- "mental models"/"pathways" participants use during the ideation exercise: 1) how can we use these partterns to better support practitioners? 2) how much does our framework incorporate some of the dimensions they are grounding their thinking in? 3) how seeing our framework influences the way they approached their own ideation process? (some of the participants did try to adopt it)
-- examples of what our participants found surprising; the framework helps them discover surprising harms/stakeholders
-- are the generated harms actionable? while some participants raise concerns about the harms not being actionable (particularly those closer to product and/or responsible for implementing mitigations) while others noted the tendency of teams to couple harms to mitigation and the value of separating the process of ideating about harms from how those harms should be mitigated. what are some design implications here that we could highlight? 
-- are the generated harms specific to the AI? can we elaborate on why this may or may not matter? these might still happen and might make stakeholder understand what type of interventions/mitigation are needed; perhaps we can say something about how the use of AI might obfuscate/make hard to mitigate/deny recourse/people trust more the system
-- the signal to noise challenge: are the generated harms actual harms? people need now to check whether the generations are actually meaningful/useful to them  
-- will a framework as ours lead to overreliance/fail to provide incentives for them to engage more deeply with the harms ideation exercise. 
-- when in the ideation process do participants think our tool will be useful? (e.g., product -- to not start with a blank page, people that have trained teams -- to use afterwards as a means of checking for blindspots)
-- why surfacing harms in a systematic way has value? to receive resources, to discourage deployment, transparency, inform mitigation
-- provides a systematic way to think about harms and ensure coverage
-- comments on the design of the framework: e.g., the use of crowds is the way to go; having the list of stakeholder is helpful 
-- face validity: the distribution of harms was sensible? did the harms they were observing made sense? 
-- presenting/communicating generated harms: opportunities/challenges -- how to group stakeholders? how to present numbers?



% Some things which might be worth surfacing here ...
% Facilitating ethical reflection about the impact of AI systems
% Challenges to building tools to facilitate ethical reflection (hard to establish ground truth for what is a harm, risk overreliance, low signal to noise ratio, not actionable, etc)
% differences in how different type of stakeholders assessed things
% when the tool can be helpful 

\subsubsection{Facilitating ethical reflection about the impact of AI systems}
All participants found \frameworkname{} valuable for brainstorming about the adverse impacts of different AI systems. They appreciated the diversity of perspectives and systemic representation of harms that the framework offers. In particular, P2 noted that our participatory design approach, which involves experimenting with crowdsourcing and large language model, is the right way to think about these tools. By bringing a diversity of voices into impact assessment, we are working towards fair and accessible technologies. 

In terms of the framework's structure, some participants remarked that AHA offers a systemic approach to thinking about harms. Notably, one of our interviewees significantly changed their brainstorming strategy after interacting with our framework. When being prompted with the first scenario, they drew on known instances of harms and only briefly talked about relevant stakeholders when asked to elaborate. After seeing the harms in our framework, however, they formulated their response to the second scenario around a list of stakeholders, resulting in a much richer list of possible harms. When asked for comments, they noted that this change was largely informed by the structure of our framework: 
\begin{displayquote} \em
I think in general this system is a really good structure and having just read a very structured approach to generating harms made it much easier to repeat that in the context of an abstract scenario. (P1 - product PM)
\end{displayquote}
Our participants also drilled down to how components of the framework (stakeholder list, harm types) can lead to a more comprehensive and productive evaluation of AI systems. They reflected on how the list of stakeholders, high-level codes, and generated harms prompted them to think about a wider range of adverse impacts. Some participants particularly appreciated having a predefined list of stakeholders. During the brainstorming section of the interview, many participants noted that they saw stakeholders that they did not consider immediately. According to P2, developers similarly spend most of the time focusing solely on their system and thus can miss many harms. When asked to brainstorm about possible stakeholders, they are more likely to default to direct stakeholders and forget about groups of people indirectly affected by the system. For example, in the \textit{Hiring} scenario, people are inclined to come up with applicants instead of family and friends of applicants. Therefore, having a predefined list of stakeholders can help practitioners notice less obvious groups and cover a more diverse range of associated harms. 

In addition to the stakeholder list, our participants also appreciated that our framework classifies the harms according to the types of system failures (false negative/positive). As P5 noted, our tool can encourage people to think about what kind of harms are more likely to result from a certain kind of system failure: 
\begin{displayquote} 
    I think it's easy to think about harms I can arise with false positives, because there are all these, you know, reputational damages and potential damages to job security. But thinking about false negative harms may be a little bit more challenging. So I think anything that helps in that sort of visualization or help in terms of you know, these are the types of that there may be more harms that is arising from false positives. It should be really carefully done to not exacerbate overlooking in one specific harm. (P5 - RAI practice) 
\end{displayquote}

Participants also reflected on the roles of \frameworkname{} in brainstorming exercises. Our framework provides a list of high-level harms, which users can quickly browse and learn more about harms of interest. According to three participants, this feature would be helpful when users have limited time or encounter a brainstorming block. When it comes to which brainstorming stage \frameworkname{} would be most helpful in, our interviewees offered two different perspectives. Some thought that our framework should come in at the first stage of brainstorming, while others prefer to use it as a secondary check after an independent brainstorming session. Participants in the first group noted that \frameworkname{} will give people with little experience in impact assessment a head start. Rather than going through a brainstorming exercise from scratch, practitioners can build their evaluation on the existing generations in our framework. According to P8, 
\begin{displayquote}
    nobody should be starting from scratch with an impact assessment... we should be building on each other's learning and understanding what's different about the nuances of my scenario or my system, not the things that we already know. (P8 - RAI policy)
\end{displayquote}
Indeed, a long-term benefit of \frameworkname{} is that it can serve as a growing repository of harms in AI systems. As suggested by P8, previous scenarios may be saved in the framework's archive and made accessible to people going through the same exercise in the future. People can then get inspiration from similar scenarios to broaden the brainstorming field for their own scenario. 

Rather than using \frameworkname{} in the first brainstorming exercise, some participants prefer to leverage it as a secondary check. By using \frameworkname{} in a later stage, developers would be deterred from overrelying on the system, which defeats the purpose of a brainstorming exercise, as noted by P4: 
\begin{displayquote}
    I would want to continue using this as sort of that secondary check because I do like forcing teams into some open world envisioning and before they have a framework that they can just lean on and check boxes and look at specific things and call it a day. (P4 - RAI practice)
\end{displayquote}
In addition to encouraging independent brainstorming, using \frameworkname{} in a later stage of evaluation can help practitioners check for blind spots. Thanks to the breadth of the generated issues, users are likely to notice harms that they haven't previously thought of. From there, they can make sure that they are focusing on the right aspects and put together a comprehensive impact assessment.

\subsubsection{\frameworkname{} provides a structured framework to make deployment decisions}
\frameworkname{} can facilitate the decision-making process during deployment. Using our framework, people can decide whether a framework is eligible for deployment and draw up a mitigation plan if necessary. According to P3, \frameworkname{} can inform the decision-making process of people on a higher seniority level: 
\begin{displayquote}
    such a system would be even, like, useful, maybe for like higher level people that are deciding you and to build a system where you could have a description and then get like a kind of a generation of different times of can come up out of deploying such a system in a while, but individual sort of people that are down in the hierarchy don't have any actionable thing to do by seeing these harms. So maybe like people that are like making these. But like calling, the shots are are the people who need to to have such a system and browse through maybe the different times that can arise even like, without starting to build the system. (P3 - RAI academic)
\end{displayquote}
P4 also endorsed this usage of \frameworkname{}. They noted that the breadth of the generated issues will give them an easier time to find evidence for or against the deployment of an AI system. P5 further specified the ideal time range for such usage of \frameworkname{}: if the framework is involved in deployment decisions, it should be used early in the development process. P5 noted: 
\begin{displayquote}
    I assume it could support the leadership and also making maybe informed decision, especially if this is being done early on in the process like before every anything is built to help them make decisions around what are the cause in terms of responsibility. (P5 - RAI practice) 
\end{displayquote}
Another use of \frameworkname{} is to support harm mitigation, which can happen at the same time as the deployment decision-making process. It is important to understand what is wrong with the system, but it is also equally important to know what we can do to fix it. Thanks to the diverse perspectives offered by the framework, users may have a better idea of which harms are actionable, and which harms are not. As noted by P3, in some cases, the data in our framework could be used to give people a sense of "how much trouble I am in" and which areas might need more resources to address the issues. 

